Intel HEXL: Accelerating Homomorphic Encryption with Intel AVX512-IFMA52

Modern implementations of homomorphic encryption (HE) rely heavily on polynomial arithmetic over a finite field. This is particularly true of the CKKS, BFV, and BGV HE schemes. Two of the biggest performance bottlenecks in HE primitives and applications are polynomial modular multiplication and the forward and inverse number-theoretic transform (NTT). Here, we introduce Intel Homomorphic Encryption Acceleration Library (Intel HEXL), a C++ library which provides optimized implementations of polynomial arithmetic for Intel processors. Intel HEXL takes advantage of the recent Intel Advanced Vector Extensions 512 (Intel AVX512) instruction set to provide state-of-the-art implementations of the NTT and modular multiplication. On the forward and inverse NTT, Intel HEXL provides up to 7.2x and 6.7x speedup, respectively, over a native C++ implementation. Intel HEXL also provides up to 6.0x speedup on the element-wise vector-vector modular multiplication, and 1.7x speedup on the element-wise vector-scalar modular multiplication. Intel HEXL is available open-source at https://github.com/intel/hexl under the Apache 2.0 license and has been adopted by the Microsoft SEAL and PALISADE homomorphic encryption libraries.

==> Makefile <==
all: intel-hexl.pdf

# CUSTOM BUILD RULES

# In case you didn't know, '$@' is a variable holding the name of the target,
# and '$<' is a variable holding the (first) dependency of a rule.
# "raw2tex" and "dat2tex" are just placeholders for whatever custom steps
# you might have.

%.tex: %.raw
	./raw2tex $< > $@

%.tex: %.dat
	./dat2tex $< > $@

# MAIN LATEXMK RULE

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.

# -interaction=nonstopmode keeps the pdflatex backend from stopping at a
# missing file reference and interactively asking you for an alternative.

intel-hexl.pdf: intel-hexl.tex
	rm -f intel-hexl.pdf && latexmk -pdf -pdflatex="pdflatex -interaction=nonstopmode" -pvc -use-make intel-hexl.tex

clean:
	rm -f intel-hexl.bbl
	latexmk -CA

check:
	aspell --lang=en --mode=tex check abstract.tex
	aspell --lang=en --mode=tex check intel-hexl.tex

	# Should have ~ instead of space before any references / citations
	cat *.tex | grep ' \\cite'
	cat *.tex | grep ' \\ref'

.PHONY: main.pdf

